BungeeNeRF: Progressive Neural Radiance Field for Extreme Multi-scale Scene Rendering

Neural radiance fields (NeRF) has achieved outstanding performance in modeling 3D objects and controlled scenes, usually under a single scale. In this work, we focus on multi-scale cases where large changes in imagery are observed at drastically different scales. This scenario vastly exists in real-world 3D environments, such as city scenes, with views ranging from satellite level that captures the overview of a city, to ground level imagery showing complex details of an architecture; and can also be commonly identified in landscape and delicate minecraft 3D models. The wide span of viewing positions within these scenes yields multi-scale renderings with very different levels of detail, which poses great challenges to neural radiance field and biases it towards compromised results. To address these issues, we introduce BungeeNeRF, a progressive neural radiance field that achieves level-of-detail rendering across drastically varied scales. Starting from fitting distant views with a shallow base block, as training progresses, new blocks are appended to accommodate the emerging details in the increasingly closer views. The strategy progressively activates high-frequency channels in NeRF's positional encoding inputs and successively unfolds more complex details as the training proceeds. We demonstrate the superiority of BungeeNeRF in modeling diverse multi-scale scenes with drastically varying views on multiple data sources (city models, synthetic, and drone captured data) and its support for high-quality rendering in different levels of detail.

==> tables/main_exp.tex <==

% \begin{table*}[t]
% \centering

% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}l@{\,\,}|c|c|c|c|c|c}
%     Scene & & \multicolumn{4}{c|}{PSNR/ per stages} \\
%     \emph{56 Leonard} & Configuration & Stage 1 & Stage 2 & Stage 3 & Stage 4 & Avg. PSNR / LPIPS / SSIM (\uparrow) \\ \hline

% NeRF& D=8, W=256, Skip=4  & & & & & \\  
% NeRFie (WPE) & D=8, W=256, Skip=4  & & & & & \\  
% % NeRF + (Attentaive PE) & D=10, W= 256, Skip=4 & & & & & \\
% Mip-NeRF (IPE) & D=8, W= 256, Skip=4 & & & & & \\
% Mip-NeRF (IPE) & D=10, W= 256, Skip=4 & & & & & \\
% Mip-NeRF (IPE) & D=10, W=256, Skip=4,6,8 & & & & & \\  
% \hline
% Ours & D_{base}=4, B=1, W=256, $W_{res}$=256 & & & & & \\
% Ours & D_{base}=4, B=2, W=256, $W_{res}$=256 & & & & & \\ 
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=256 & & & & & \\  
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=128 & & & & & \\  
% Ours & D_{base}=6, B=3, W=256, $W_{res}$=256 & & & & & \\  
% \midrule
% Ours (Best) & & & & & & \\  
% \bottomrule
% \end{tabular}
% }

% \caption{Main Comparison Experiments on 1) \emph{56 Leonard (NYC)} scene and 2) \missref scene.}
% \label{tab:main_exp_tmp}
% \end{table*}


\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|cccc|c|}
\hline
\multirow{2}{*}{}                           & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Configuration}} & \multicolumn{4}{c|}{\textbf{PSNR / scale}}                                                           & \multirow{2}{*}{\textbf{avg. PSNR/LPIPS/SSIM}} \\ \cline{4-7}
                                            &                                 &                                         & \multicolumn{1}{c|}{L=1}     & \multicolumn{1}{c|}{L=2}     & \multicolumn{1}{c|}{L=3}     & L=4     &                                                \\ \hline
\multirow{4}{*}{\textbf{General baselines}} & NeRF                            & \multirow{3}{*}{D=8, Skip=4}     & \multicolumn{1}{c|}{21.2789} & \multicolumn{1}{c|}{22.0534} & \multicolumn{1}{c|}{22.0997} & 21.8532 & 21.7019/ 0.3206/ 0.6355                        \\ \cline{2-2} \cline{4-8} 
                                            & nerfies (WPE)                   &                                         & \multicolumn{1}{c|}{22.0220} & \multicolumn{1}{c|}{22.0968} & \multicolumn{1}{c|}{21.7993} & 21.4390 & 21.6724/ 0.3648/ 0.6325                        \\ \cline{2-2} \cline{4-8} 
                                            & MipNeRF (IPE)                   &                                         & \multicolumn{1}{c|}{21.8993} & \multicolumn{1}{c|}{22.1792} & \multicolumn{1}{c|}{22.0454} & 21.7632 & 21.9754/ 0.3440/ 0.6476                        \\ \cline{2-8} 
                                            & MipNeRF (IPE)                   & D=10, Skip=4                     & \multicolumn{1}{c|}{22.0196} & \multicolumn{1}{c|}{22.4025} & \multicolumn{1}{c|}{22.2774} & 21.9749 & 22.2273/ 0.3183/ 0.6660                        \\ \hline
\textbf{Static w/ full skip layer}          & MipNeRF (IPE)                   & D=10, Skip=4,6,8                 & \multicolumn{1}{c|}{22.0432} & \multicolumn{1}{c|}{22.4840} & \multicolumn{1}{c|}{22.6897} & 22.3552 & 22.3123/ 0.2663/ 0.6897                        \\ \hline
\textbf{Ours (Best)}                        &                                 &                                         & \multicolumn{1}{c|}{23.1451} & \multicolumn{1}{c|}{23.5483} & \multicolumn{1}{c|}{23.7440} & 23.0154 & 23.4810/ 0.2347/ 0.7394                        \\ \hline
\textbf{Ours (Longer Time)}                 &                                 &                                         & \multicolumn{1}{c|}{24.0824}        & \multicolumn{1}{c|}{25.5595}        & \multicolumn{1}{c|}{25.4762}        & 25.2618 & 24.6302/ 0.1588/ 0.8179       \\ \hline
\end{tabular}
}
\caption{Main Comparison Experiments on \emph{56 Leonard (NYC)} scene.}
\label{tab:main_exp}
\end{table*}

\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|cccc|c|}
\hline
\multirow{2}{*}{}                           & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Configuration}} & \multicolumn{4}{c|}{\textbf{PSNR / stage}}                                                           & \multirow{2}{*}{\textbf{avg. PSNR/LPIPS/SSIM}} \\ \cline{4-7}
                                            &                                 &                                         & \multicolumn{1}{c|}{Stage1}  & \multicolumn{1}{c|}{Stage2}  & \multicolumn{1}{c|}{Stage3}  & Stage4  &                                                \\ \hline
\multirow{4}{*}{\textbf{General baselines}} & NeRF                            & \multirow{3}{*}{D=8, W=256, Skip=4}     & \multicolumn{1}{c|}{22.7110} & \multicolumn{1}{c|}{22.8110} & \multicolumn{1}{c|}{22.9756} & 21.5806 & 22.6420/ 0.3175/0.6901                         \\ \cline{2-2} \cline{4-8} 
                                            & nerfies (WPE)                   &                                         & \multicolumn{1}{c|}{23.3817} & \multicolumn{1}{c|}{23.1714} & \multicolumn{1}{c|}{22.4496} & 20.8056 & 22.3516/ 0.3308/ 0.6797                        \\ \cline{2-2} \cline{4-8} 
                                            & MipNeRF (IPE)                   &                                         & \multicolumn{1}{c|}{23.3461} & \multicolumn{1}{c|}{23.0298} & \multicolumn{1}{c|}{22.6449} & 20.9368 & 22.6919/ 0.3270/ 0.6874                        \\ \cline{2-8} 
                                            & MipNeRF (IPE)                   & D=10, Skip=4                     & \multicolumn{1}{c|}{23.1964} & \multicolumn{1}{c|}{22.8997} & \multicolumn{1}{c|}{22.4394} & 20.7428 & 22.5253/ 0.3298/ 0.6864                        \\ \hline
\textbf{Static w/ full skip layer}          & MipNeRF (IPE)                   & D=10, Skip=4,6,8                 & \multicolumn{1}{c|}{23.3773} & \multicolumn{1}{c|}{23.1563} & \multicolumn{1}{c|}{22.8544} & 21.1516 & 22.8284/ 0.3138/ 0.6986                        \\ \hline
\textbf{Ours (Best)}                        &                                 &                                         & \multicolumn{1}{c|}{24.2590} & \multicolumn{1}{c|}{23.9110} & \multicolumn{1}{c|}{23.5072} & 22.9417 & 23.6055/ 0.2652/ 0.7487                        \\ \hline
\textbf{Ours (Longer Time)}                 &                                 &                                         & \multicolumn{1}{c|}{24.5133} & \multicolumn{1}{c|}{24.5410} & \multicolumn{1}{c|}{24.5025} & 23.6398 & 24.3934/ 0.1933/ 0.7998                        \\ \hline
\end{tabular}
}
\caption{Main Comparison Experiments on \emph{Transamerica Pyramid} scene.}
\label{tab:main_exp}
\end{table*}


\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|cccc|c|}
\hline
\multirow{2}{*}{}        & \multicolumn{4}{c|}{\textbf{PSNR / scale}}                                                           & \multirow{2}{*}{\textbf{avg. PSNR/LPIPS/SSIM}} \\ \cline{2-5}
                         & \multicolumn{1}{c|}{L=1}     & \multicolumn{1}{c|}{L=2}     & \multicolumn{1}{c|}{L=3}     & L=4     &                                                \\ \hline
\textbf{w/o skip layer}  & \multicolumn{1}{c|}{23.0466} & \multicolumn{1}{c|}{23.3640} & \multicolumn{1}{c|}{23.3173} & 22.7463 & 23.1588/ 0.2594/ 0.7295                        \\ \hline
\textbf{w/o residual}    & \multicolumn{1}{c|}{23.1037} & \multicolumn{1}{c|}{23.3257} & \multicolumn{1}{c|}{23.2282} & 22.7858 & 23.1385/ 0.2569/ 0.7290                        \\ \hline
\textbf{w/o multi-level sup.}  & \multicolumn{1}{c|}{22.5700} & \multicolumn{1}{c|}{22.4753} & \multicolumn{1}{c|}{23.3001} & 23.1885 & 22.7729/ 0.2976/ 0.7004                        \\ \hline
\textbf{w/o multi-step data feeding} & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &         &                                                \\ \hline
\textbf{w/o model growing} & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &         &                                                \\ \hline
\end{tabular}
}
\caption{Ablation study on \emph{56 Leonard (NYC)} scene.}
\label{tab:ablate_56leonard}
\end{table}

\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|cccc|c|}
\hline
\multirow{2}{*}{}       & \multicolumn{4}{c|}{\textbf{PSNR / scale}}                                                           & \multirow{2}{*}{\textbf{avg. PSNR/LPIPS/SSIM}} \\ \cline{2-5}
                        & \multicolumn{1}{c|}{L=1}     & \multicolumn{1}{c|}{L=2}     & \multicolumn{1}{c|}{L=3}     & L=4     &                                                \\ \hline
\textbf{w/o skip layer} & \multicolumn{1}{c|}{24.2328}        & \multicolumn{1}{c|}{23.6975}        & \multicolumn{1}{c|}{22.9501}        & 22.1512 & 23.2349/ 0.2831/ 0.7245                                             \\ \hline
\textbf{w/o residual}   & \multicolumn{1}{c|}{24.0919} & \multicolumn{1}{c|}{23.6075} & \multicolumn{1}{c|}{23.2364} & 22.7956 & 23.3638/ 0.2721/ 0.7354                        \\ \hline
\end{tabular}
}
\caption{Ablation study on \emph{Transamerica Pyramid} scene.}
\label{tab:ablate_transamerica}
\end{table}


\begin{table*}[t]
\centering

\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
                                     & \multicolumn{4}{c|}{\textbf{Configuration}}                                                      & \multicolumn{4}{c|}{\textbf{PSNR/ per stages}}        &                                                     \\ \cline{2-9}
\multirow{-2}{*}{}                   & D\_Base & B                         &  Skip Layer                    & Header                       & Stage 1 & Stage 2 & Stage 3                 & Stage 4 & \multirow{-2}{*}{\textbf{avg. PSNR / LPIPS / SSIM}} \\ \hline
\textbf{Ours (Best)}                 & 4       & 3                         & 4,6,8                        & Residual                     &         &         &                         &         &                                                     \\ \hline
                                     & 4       & \cellcolor[HTML]{FFFE65}2 & 4,6,8                         & Residual                     &         &         &                         &         &                                                     \\ \cline{2-10} 
\multirow{-2}{*}{\textbf{\# Blocks}} & 4       & \cellcolor[HTML]{FFFE65}1 & 4,6,8                         & Residual                     &         &         & {\color[HTML]{000000} } &         &                                                     \\ \hline
\textbf{w/o Skip Layer per block}           & 4       & 3                         & \cellcolor[HTML]{FFCC67}4 & Residual                     &         &         &                         &         &                                                     \\ \hline
\textbf{\# Header}                   & 4       & 3                         & 4,6,8                         & \cellcolor[HTML]{68CBD0}Full &         &         &                         &         &                                                     \\ \hline
\end{tabular}

% \begin{tabular}{@{}l@{\,\,}|c|c|c|c|c|c}
%     Scene & & \multicolumn{4}{c|}{PSNR/ per stages} \\
%     \emph{56 Leonard} & Configuration & Stage 1 & Stage 2 & Stage 3 & Stage 4 & Avg. PSNR / LPIPS / SSIM (\uparrow) \\ \hline
% Ours & D_{base}=4, B=1, W=256, $W_{res}$=256 & & & & & \\
% Ours & D_{base}=4, B=2, W=256, $W_{res}$=256 & & & & & \\ 
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=256 & & & & & \\  
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=128 & & & & & \\  
% Ours & D_{base}=6, B=3, W=256, $W_{res}$=256 & & & & & \\  
% \end{tabular}
}

\caption{Ablation study on 1) \emph{56 Leonard (NYC)} scene and 2) \missref scene.}
\label{tab:ablate_exp}
\end{table*}

% \vspace{25pt}

% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}l@{\,\,}|c|c|c|c|c|c}
%     Scene & & \multicolumn{4}{c|}{PSNR/ per stages} \\
%     [TBD] & Configuration & Stage 1 & Stage 2 & Stage 3 & Stage 4 & Avg. PSNR / LPIPS / SSIM (\uparrow) \\ \hline

% NeRF & D=10, W=256, Skip=4  & & & & & \\  
% NeRF + WPE & D=10, W=256, Skip=4  & & & & & \\  
% % NeRF + (Attentaive PE) & D=10, W= 256, Skip=4 & & & & & \\
% Mip-NeRF (IPE) & D=10, W= 256, Skip=4 & & & & & \\
% Mip-NeRF (IPE) & D=10, W=256, Skip=4,6,8 & & & & & \\  
% \hline
% Ours & D_{base}=4, B=1, W=256, $W_{res}$=256 & & & & & \\
% Ours & D_{base}=4, B=2, W=256, $W_{res}$=256 & & & & & \\ 
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=256 & & & & & \\  
% Ours & D_{base}=4, B=3, W=256, $W_{res}$=128 & & & & & \\  
% Ours & D_{base}=6, B=3, W=256, $W_{res}$=256 & & & & & \\  
% \midrule
% Ours (Best) & & & & & & \\  
% \bottomrule
% \end{tabular}
% }



==> tables/single_scale_average.tex <==
NeRF (Jax Impl.)~\cite{jaxnerf2020github,mildenhall2020} &                    31.74 &                    0.953 &                    0.050 &                    0.0194 & $3.05 \pm 0.01$ & 1,191\thousand \\
NeRF + Centered Pixels                                            &                    32.30 &                    0.957 &                    0.046 &                    0.0178 & $2.99 \pm 0.06$ & 1,191\thousand \\
NeRF + Center, Misc.                                              &                    32.28 &                    0.957 &                    0.046 &                    0.0178 & $3.06 \pm 0.03$ & 1,191\thousand \\
\hline
\shortmodelname                                                   & \cellcolor{red}    33.09 & \cellcolor{red}    0.961 & \cellcolor{red}    0.043 & \cellcolor{red}    0.0161 & $2.89 \pm 0.00$ & 612\thousand \\
\shortmodelname w/o Misc.                                         & \cellcolor{orange} 33.04 & \cellcolor{orange} 0.960 & \cellcolor{red}    0.043 & \cellcolor{red}    0.0162 & $2.89 \pm 0.01$ & 612\thousand \\
\shortmodelname w/o Single MLP                                    & \cellcolor{yellow} 32.71 & \cellcolor{yellow} 0.959 & \cellcolor{orange} 0.044 & \cellcolor{orange} 0.0168 & $3.63 \pm 0.02$ & 1,191\thousand \\
\shortmodelname w/o \shortfeaturename                             &                    32.48 &                    0.958 & \cellcolor{yellow} 0.045 & \cellcolor{yellow} 0.0173 & $2.84 \pm 0.00$ & 612\thousand \\

